MUDGUARD: Taming Malicious Majorities in Federated Learning using Privacy-Preserving Byzantine-Robust Clustering

Byzantine-robust Federated Learning (FL) aims to counter malicious clients and train an accurate global model while maintaining an extremely low attack success rate. Most existing systems, however, are only robust when most of the clients are honest. FLTrust (NDSS '21) and Zeno++ (ICML '20) do not make such an honest majority assumption but can only be applied to scenarios where the server is provided with an auxiliary dataset used to filter malicious updates. FLAME (USENIX '22) and EIFFeL (CCS '22) maintain the semi-honest majority assumption to guarantee robustness and the confidentiality of updates. It is therefore currently impossible to ensure Byzantine robustness and confidentiality of updates without assuming a semi-honest majority. To tackle this problem, we propose a novel Byzantine-robust and privacy-preserving FL system, called MUDGUARD, that can operate under malicious minority \emph{or majority} in both the server and client sides. Based on DBSCAN, we design a new method for extracting features from model updates via pairwise adjusted cosine similarity to boost the accuracy of the resulting clustering. To thwart attacks from a malicious majority, we develop a method called \textit{Model Segmentation}, that aggregates together only the updates from within a cluster, sending the corresponding model only to the clients of the corresponding cluster. The fundamental idea is that even if malicious clients are in their majority, their poisoned updates cannot harm benign clients if they are confined only within the malicious cluster. We also leverage multiple cryptographic tools to conduct clustering without sacrificing training correctness and updates confidentiality. We present a detailed security proof and empirical evaluation along with a convergence analysis for MUDGUARD.

==> sections/cryptotools.tex <==
\section{Other Cryptographic Tools}
\label{sec:cryptotools}

\noindent\textbf{Homomorphic Encryption (HE).}
This tool is an interesting privacy-preserving technology enabling users to evaluate polynomial computations on ciphertexts without revealing underlying plaintexts. 
An encryption scheme is called partial HE if it only supports addition~\cite{paillier1999public} or multiplication~\cite{elgamal1985public}, while fully HE~\cite{gentry2009fully} may support both. 
An HE scheme usually includes the following steps. \\
%\begin{itemize}
$\bullet$ \textit{Key Generation:} $(\pk ,\sk)$ $\leftarrow \kgen$ ($1^\lambda$), where based on security level parameter $\lambda$, public key $\pk$ and secret key $\sk$ can be generated.\\
$\bullet$ \textit{Encryption:} $(c_1, c_2) \leftarrow \enc(\pk, m_1, m_2)$. By using $\pk$, the probabilistic algorithm encrypts messages $m_1, m_2$ to ciphertexts $c_1, c_2$.\\
$\bullet$ \textit{Homomorphic evaluation:} $\eval(c_1, c_2)=c_1\circ c_2=\enc(\pk,m_1)\circ \enc(\pk, m_2)=\enc(\pk, m_1\circ m_2)$, where $\circ$ refers to an operator, e.g., addition or multiplication. \\
$\bullet$ \textit{Decryption:} $m_1\circ m_2\leftarrow \dec(\sk, \enc(\pk, m_1\circ m_2))$. Using $\sk$, the operational results of $m_1$ and $m_2$ can be derived.

\noindent\textbf{Oblivious Transfer (OT).} OT~\cite{rabin2005exchange} is one of the crucial building blocks for MPC. 
In an OT protocol (involving two parties), a sender holds $n$ different strings $s_i, i=1\cdots n,$ and a receiver has an index ($ind$) and wants to learn $s_{ind}$. 
At the end of the protocol, the receiver cannot get information about strings rather than $s_{ind}$, while the sender learns nothing about $ind$ selected by the receiver. 
For example, 
%Instantiatedly\todo{?},
a 1-out-of-2 OT protocol only inputs two strings and a 1-bit index. 

\noindent{\textbf{Garbled Circuits (GC)~\cite{bellare2012foundations}.}} The protocol is run between two parties called the garbler and evaluator. The garbler generates the GC corresponding to the Boolean circuit to be evaluated securely by associating two random keys per wire representing the bit values {0, 1}. The garbler then sends the GC together with the keys for the inputs to the evaluator. The evaluator obliviously obtains the keys for his inputs via OT and evaluates the circuit to obtain the output key. Finally, the evaluator maps the output key to the real output.
